Reinforcement Learning with Token-level Feedback for Controllable Text Generation

To meet the requirements of real-world applications, it is essential to control generations of large language models (LLMs). Prior research has tried to introduce reinforcement learning (RL) into controllable text generation while most existing methods suffer from overfitting issues (finetuning-based methods) or semantic collapse (post-processing methods). However, current RL methods are generally guided by coarse-grained (sentence/paragraph-level) feedback, which may lead to suboptimal performance owing to semantic twists or progressions within sentences. To tackle that, we propose a novel reinforcement learning algorithm named TOLE which formulates TOken-LEvel rewards for controllable text generation, and employs a "first-quantize-then-noise" paradigm to enhance the robustness of the RL algorithm.Furthermore, TOLE can be flexibly extended to multiple constraints with little computational expense. Experimental results show that our algorithm can achieve superior performance on both single-attribute and multi-attribute control tasks. We have released our codes at https://github.com/WindyLee0822/CTG

==> latex/sections/abstract.tex <==
\begin{abstract}

To meet the requirements of real-world applications, it is essential to control generations of large language models (LLMs). 
Prior research has tried to introduce reinforcement learning (RL) into controllable text generation while most existing methods suffer from overfitting issues (finetuning-based methods) or semantic collapse (post-processing methods). 
However, current RL methods are generally guided by coarse-grained (sentence/paragraph-level) feedback, which may lead to suboptimal performance owing to semantic twists or progressions within sentences.
To tackle that, we propose a novel reinforcement learning algorithm named \textbf{TOLE} which formulates \textbf{TO}ken-\textbf{LE}vel rewards for controllable text generation, and employs a "first-quantize-then-noise" paradigm to enhance the robustness of the RL algorithm.   
Furthermore, TOLE can be flexibly extended to multiple constraints with little computational expense. 
Experimental results show that our algorithm can achieve superior performance on both single-attribute and multi-attribute control tasks. We have released our codes at \url{https://github.com/WindyLee0822/CTG}.
\end{abstract}

==> latex/sections/conclusion.tex <==
\section{Conclusion}
To summarize, we propose an extensible reinforcement learning algorithm for controllable text generation with token-level feedback. We provide an alternative perspective of Bayesian Factorization, which enlightens our token-level reward design. We also introduce "Quantization \& Noise" into RL to enhance the algorithm robustness. We also propose a small-scale module "weigher" to extend our algorithm to multiple constraints. Extensive experiments demonstrates the effectiveness of our algorithm.

\section*{Limitations}
First, our algorithm cannot achieve 100\% accuracies in the vast majority of aspects (e.g., sentiment or topic), which may be not acceptable in scenarios with requirements of 100\% control fulfillment. 
Second, although extensive experiments have been conducted to demonstrate the effectiveness of our algorithm, applying it to more LLM structures can verify the generalizability of \textsc{Tole}. 
Third, our approach is limited in the attribute control task so far, and may be hard to apply our algorithm to
other scenarios e.g., lexical constraint, table-to-text. However, most current research on CTG generally focuses on attribute control tasks, and shares this limitation, which is an open problem that should be explored in future works.

\section*{Ethics Statement}
Since the large language models (LLMs) are trained on data collected from the web and often not thoroughly
cleaned, they can generate offensive or toxic text. We
must state that the texts generated by our approach
do not represent our opinion. However, our experiments show that our algorithms can handle the detoxification tasks which can alleviate the toxic degeneration problems of LLMs. Moreover, the extensibility of our model can extend the detoxification tasks to all control requirements by taking it as an additional constraint.  

\section*{Acknowledgement}
This work was supported in part by the National Natural Science Foundation of China under Grant No. 62276110, No. 62172039 and in part by the fund of Joint Laboratory of HUST and Pingan Property \& Casualty Research (HPL). The authors would also like to thank the anonymous reviewers for their comments on improving the quality of this paper. 


==> latex/sections/experiments.tex <==
\section{Experiments}
\label{sec:exp}

\begin{table*}[t!]
    \centering\footnotesize
    \tabcolsep=3pt
    \renewcommand\arraystretch{1.1}
    \begin{adjustbox}{max width=1\linewidth,width=0.95\linewidth,center=\linewidth}
    \begin{tabular}{cc|cc|cc|ccc|c}
    \toprule
      \multirow{3}{*}{\textbf{Category}}  & \multirow{3}{*}{\textbf{Model}} & \multicolumn{4}{c|} {\textbf{Attribute Correctness}($\uparrow$)} & \multicolumn{3}{c|}{\textbf{Generation Metrics} }& {\textbf{Training Info.} } \\ 
      \cmidrule{3-10}
        &&\multicolumn{2}{c|}{\textbf{Target}:\textsc{Positive}} &\multicolumn{2}{c|}{\textbf{Target}:\textsc{Negative}} &  \multirow{2}{*}{\quad PPL($\downarrow$)}  & \multirow{2}{*}{dist-3($\uparrow$)}& \multirow{2}{*}{CR.($\downarrow$)} & \multirow{2}{*}{\%Params} \\
        && negative & neutral & positive & neutral & &  & \\
          \midrule
          \midrule
        % &GPT2 & \phantom{0}0.00 & 50.02 & 11.42 & 50.02 & 11.42 & 0.84 & 0.84 & - \\
        % \midrule
        \multirow{3}{*}{\makecell[c]{Post-\\processing}}&PPLM & \phantom{0}8.72 & 52.68 & 10.26 & 60.95 & 122.41 & \textbf{0.90 } &3.47&  0.001   \\
        &\textsc{GeDi} & 26.80 & 86.01 & 60.43 & 91.27 &138.27&\underline{0.86}& 3.62&-  \\
        %DExpert & 36.42 & 94.46 & 64.01 & 96.23 & 67.12 & 0.64 & 0.83 & - &\\
        &FUDGE & 56.04 & 96.92 & 66.84 & \textbf{98.76} & 265.79 & 0.83& 1.53& - \\    
        \midrule
         \multirow{2}{*}{\makecell[c]{Fine-\\Tuning}}&\textsc{Prompt} & 40.88 & 78.08 & 49.28 & 73.20 & 39.55  & 0.73 & 63.08 &0.003    \\
        &\textsc{DisCup} & \underline{49.92}& 91.58  & 60.80 &90.64 & 40.46 & 0.75 & 3.72 & 0.003  \\
        \midrule
        \multirow{3}{*}{\makecell[c]{Reinforcement\\Learning}} &PPO  & 43.13 & 94.10 & 68.12 & 94.95 & 18.34  & 0.71& 2.95 & 100 \\
        &\textsc{Quark}  & 47.32& \underline{95.50} & \underline{70.50} & 96.65 & \textbf{16.92} & 0.75& 2.63 & 100  \\
        \cmidrule{2-10}
        &TOLE & \textbf{69.36} & \textbf{97.16}& \textbf{72.81} &  \underline{98.02} & \underline{17.05} & 0.75 &2.61 & 0.003  \\
    \bottomrule
    \end{tabular}
    \end{adjustbox}
    \caption{Automatic evaluation results of the sentiment control task. "Params" indicates the ratio of trainable parameters to the whole LLM. Boldface and underline indicate the best two results.}
    \label{tab:sentiment}
\end{table*}

% \begin{table*}[t!]
%     \centering
%     \tabcolsep=5pt
%     \renewcommand\arraystretch{1.0}
%     \begin{adjustbox}{max width=1\linewidth,width=0.95\linewidth,center=\linewidth}
%     \begin{tabular}{cc|cccc|ccc}
%     \toprule
%       \multirow{2}{*}{\textbf{Category}} &  \multirow{2}{*}{\textbf{Model}} & \multicolumn{4}{c|} {\textbf{Repetition}}  & \multicolumn{3}{c}{\textbf{Text Quality} } \\ \cmidrule{3-9}
%     && rep-2$(\downarrow)$  & rep-3$(\downarrow)$ & rep-4$(\downarrow)$ & div.$(\uparrow)$ & MAUVE$(\uparrow)$ &  acc$(\uparrow)$ & coherence$(\uparrow)$  \\
%         \midrule
%         \multirow{3}{*}{\makecell[c]{Retrain \\ LLMs}} & MLE & 69.21 & 65.18& 62.05& 0.04& 0.03 & 39.63 & 0.587\\
%        & Unlikelihood & 24.12 & \textbf{13.35}& \textbf{8.04}& \textbf{0.61}& 0.69 & 38.41 & 0.568\\
%         &SimCTG &  67.36 & 63.33& 60.17 &0.05 & 0.05 & 40.91 & 0.610\\
%     \midrule
        
%         \multirow{2}{*}{\makecell[c]{ Steer \\ LLMs}} & \textsc{Quark} & 39.89 &30.62&  26.52 & 0.35 & 0.74 & 41.57 & 6.7\\
%         \cmidrule{2-9}
%         & Ours & \textbf{23.92} & 16.39 & 12.35 & 0.56 & \textbf{0.78} & 6.3 & 6.5  \\
%     \bottomrule 
%     \end{tabular}
%     \end{adjustbox}
%     \label{tbl:repetition}
%     \caption{Evaluation results of unlearning repetition. Bold numbers indicate the best performance.}
%     \label{tab:repetition}
% \end{table*}

\subsection{Sentiment Control}

\textbf{Experimental Settings.} Following previous works, we use 10K naturally occurring prompts from the OpenWebText Corpus, which is divided into 5K “neutral” prompts, 2.5K “negative” prompts, and 2.5K “positive” prompts. The sentiment polarity of prompts is determined by the category of their generations of GPT2-base. 
%The controlling task is to steer LLMs to generate sentences satisfying a different sentiment rather than the sentiment polarity of prompts.
%To inherit the ability of pre-trained language models (PLM) and reduce computational resources, we adopt prompt techniques rather than tuning the whole parameters of LMs. The parameters in the original PLM are frozen and we only train the control prompts to steer model behaviors. 
%Following \citeauthor{discup}, an LSTM module is introduced to make the control prompts close to the natural language. 
We use GPT2-large as the base PLM, and adopt prompt techniques rather than tuning the whole model. 
The sentiment scorer is based on GPT2-base, which is trained on SST-5 following \citeauthor{discup}. 
%Our scale of parameters to be updated is much smaller than prior RL methods, similar to prior prompts-based methods. 
\textit{PPL}, \textit{Dist-n} are adopted to measure the fluency and diversity of generation. \textit{Correctness} is the proportion of generations that satisfy target sentiment. We use a Huggingface sentiment classifier\footnote{\url{https://huggingface.co/
distilbert-base-uncased-finetuned-sst-2-english}} to discriminate categories of generations. See more details in Appendix \ref{apd:exp-single}.
We also conduct human evaluations based on the perceived level of sentiment correctness, topicality, and fluency. Details of human evaluation can be found in Appendix \ref{apd:human}.


\textbf{Baselines.}
A wide range of competitive baselines are compared with our algorithm.
We compare our methods to post-processing methods as follows: \textit{PPLM} \citep{pplm},\textit{GEDI} \citep{gedi}, and \textit{FUDGE} \citep{fudge}.
We also choose several competitive finetuning-based methods as our baselines:
\textit{Prompt-tuning} \citep{continuous_prompt}, \textit{DisCup} \citep{discup}.
To compare with RL-based methods, we implement \textit{PPO} \citep{PPO} and \textit{QUARK} \citep{quark}.
See more details in Appendix \ref{apd:exp-single}.

\textbf{Results and Analysis.}
The automatic evaluation results are shown in Table \ref{tab:sentiment}. 
Though post-processing can make generated sentences satisfy the target sentiment with the least parameters to train, even in a zero-shot way by decoding-time regulation with attribute discriminators, they generally get high PPL scorers, which means the quality of generated texts is poor. 
Fine-tuning methods can maintain text fluency while getting considerable accuracy of target attributes, but they suffer from overfitting the training corpus with high coverage rates. 
DisCup borrows RL paradigms by exploring candidate tokens to alleviate the overfitting problem, alleviating the overfitting issue.
RL-based methods get the best performance among all baselines. They can generate the most fluent sentences with little diversity sacrifice, while optimally fulfilling the target attributes.
Since prior RL-based methods only adopt sentence-level feedback, they can only achieve suboptimal performance even with all parameters of LLMs to be updated.
Our method guides LLMs with finer-grained feedback, thus attaining better performance with a substantial reduction of computational expenses, since it requires fewer parameters and training steps (\S \ref{sec:further_study}).
%Post-processing methods show impressive controllability, especially DExpert and Fudge which show comparable performance to finetuning or RL-based methods by regulating the possibility distribution of LMs. However, the direct manipulation of the possibility distribution causes the highest PPL scores, which indicates low text fluency. 
%We collect the generated sentences output by post-processing models in Appendix \ref{}, which shows that post-processing models often destroy the syntax structure and just repeat words expressing the target sentiment e.g. (--). It validates that post-processing words can hardly take an insight into the attribute-specific texts. 
% For finetuning methods, vanilla prompt-tuning methods like Tailor only achieve narrow performance and cause overfitting towards the training corpus, as shown that the Tailor gets the highest coverage rate among baselines. DisCup borrows RL paradigms by exploring candidate tokens to alleviate the overfitting problem, getting a performance surge among prompt-based methods. 
% Among RL-based methods, our fine-grained signals result in the best performance. Original sentence-level signals cannot provide clear guidance, leading to lower performance and tardy convergence as shown in \S\ref{sec:exp-further}. Human evaluation results and analysis are shown in Appendix \ref{apd:human_results}.
% It is noteworthy that FIRE only requires 10$\times$ fewer prefixes to achieve superior performance within 50k learning steps compared to 85k prefixes and more than 10w learning steps for 2 RL baselines.

% \subsection{Unlearn Repetition}

% \textbf{Experimental Settings.}
% Neural language models often generate repetitive, uninformative, and dull text, known as the \textit{degeneration} problem. In this part of the experiments, our objective is to unlearn repetition of LLMs. We use WIKITEXT-103 \citep{wikitext} as the dataset following \citeauthor{simctg}, which contains 1.8 million sentences from Wikipedia articles. During the evaluation, we adopt greedy decoding since degenerate repetition tends to appear most frequently with greedy decoding. 
% We use GPT2 as the base PLM and finetune the whole parameter as baselines.
% we report rep-n which measures the sequence-level repetition as the portion of duplicate n-grams in the generated text, and diversity (div.) which assesses the overall degeneration with a fusion of different n-gram levels, MAUVE \citep{mauve} which measures how much the generated text distribution diverges from that of human-written text, and PPL for text fluency.
% See more details in Appendix \ref{}.

% \textbf{Baselines.}
% Prior research tries to manage text degeneration by proposing new training objectives to substitute maximum likelihood estimation (MLE) training. We involve basic MLE training, unlikelihood training \citep{unlikelihood}, and contrastive training \citep{simctg} as our baselines. We also compare with sentence-level RL methods PPO \cite{PPO} and Quark \cite{quark}. See details in Appendix \ref{}.

% \textbf{Results and Analysis.}

\begin{table*}[t!]
    \centering\footnotesize
    \renewcommand\arraystretch{1}
    \begin{adjustbox}{max width=1\linewidth,width=0.95\linewidth,center=\linewidth}
    \begin{tabular}{l|cc|cc|cc|cc}
    \toprule
      \hspace{5.5mm}\multirow{4}{*}{\textbf{Model}} & \multicolumn{4}{c|}{ \textbf{In-domain} \textsc{RealToxicityPrompts} } & \multicolumn{4}{c}{\textbf{Out-of-domain} \textsc{WritingPrompts}} \\ \cmidrule{2-9}
        &\multicolumn{2}{c|}{\textbf{Toxicity} ($\downarrow$)} & \multicolumn{2}{c|}{\textbf{Generation}} &\multicolumn{2}{c|}{\textbf{Toxicity} ($\downarrow$)} & \multicolumn{2}{c}{\textbf{Generation}}\\
         & avg.~max. & prob. & PPL $\downarrow$ & dist-3$\uparrow$ & avg.~max. & prob. &  PPL$\downarrow$  & dist-3$\uparrow$ \\\midrule
        GPT2  & 0.527 & 0.520 & 11.31  & 0.85 & 0.572 & 0.610 & 12.99 & 0.85 \\
        \midrule
        PPLM  & 0.520 & 0.518 & 32.58  & \textbf{0.86} & 0.544 & 0.590 & 36.20  & \textbf{0.86} \\
        GeDi  & 0.363 & 0.217 & 60.03 &  0.83 & \underline{0.261} & \textbf{0.050} & 91.16 &  0.82 \\
        DExpert & 0.314 & 0.128 & 32.41  & 0.84 & 0.343 & 0.156 & 42.53  & 0.85 \\
        Prompt  & 0.302 & 0.360 & 29.21 & 0.74 & 0.442 & 0.363 & 30.10 & 0.79 \\
        Discup  & 0.298 & 0.115 & 39.30  & 0.84 & 0.442 & 0.363 & 37.23  & 0.85 \\
        PPO  & 0.288 & 0.130 & 18.22 & 0.82 & 0.291 & 0.132 & 18.32  & 0.84\\
         Quark   & \underline{0.237} & \underline{0.118} & \underline{17.23} & 0.81 & 0.268 & 0.102 & 17.19  & 0.83\\
        \midrule
        TOLE & \textbf{0.206} & \textbf{0.105} & \textbf{15.45}  & 0.80 & \textbf{0.223} & \underline{0.080} & \textbf{16.51}  & 0.83\\
    \bottomrule
    \end{tabular}
    \end{adjustbox}
    \caption{Automatic evaluation results of unlearning toxicity experiments. Boldface and underline indicate the best two results.}
    \label{tab:toxicity_results}
\end{table*}
\subsection{Detoxification}

\textbf{Experimental Settings.}
Toxic degeneration is an inherent problem of LLMs, since LLMs may express harmful or offensive utterances. 
We train the classifier on Toxicity Classification Kaggle challenge\footnote{\url{https://bit.ly/3cvG5py}}, which includes 160K toxic comments and 1.4M nontoxic comments.
We use \textsc{Real}\textsc{Toxicity}\textsc{Prompts} \cite{realtoxic} dataset as our experimental corpus which consists of 100k prompts designed to elicit toxicity. We use the 10K non-toxic test prompts following \citet{dexpert}, and take other prompts as the exploration prefixes.
We use the same LSTM-based prompt techniques on GPT2-large.
Additionally, we also conduct out-of-domain
evaluation with the \textsc{WritingPrompts} dataset \cite{writingprompts}, which is created for creative writing.
We evaluate the detoxification ability by the average maximum toxicity over 25 text generations, and the probability of at least one of any 25 generations being toxic. The toxicity is judged by Perspective API. 
We also evaluate the text quality by PPL and dist-n. See more details in \ref{apd:exp-multiple-attribute}.
We also conduct human evaluations on control accuracy, fluency, and overall text quality. The evaluation settings and results are in Appendix \ref{apd:human}.

\textbf{Baselines.}
As sentiment control tasks, we compare our methods to post-processing methods, finetuning-based methods, and RL-based methods. Post-processing methods are as follows: \textit{PPLM} \citep{pplm},\textit{GEDI} \citep{gedi}, \textit{DExpert} \citep{dexpert},.
We choose \textit{DisCup} \citep{discup} to represent finetuning-based methods.
We implement RL-based methods: \textit{PPO} \citep{PPO} and \textit{QUARK} \citep{quark}. 
See more details in Appendix \ref{apd:exp-single}.

\textbf{Results and Analysis.}
Post-processing methods get the highest PPL score, which means generated sentences are disfluent though have high diversity. 
Finetuning-based methods have ordinary performances since fine-tuning models on specific corpus is easily overfitted to undesired attributes.
RL-based methods generally achieve the lowest toxicity on both toxicity metrics. Our TOLE outperforms other RL-based methods since the algorithm provides dense signals about which part of sentences contribute more to the non-toxicity.


\subsection{Multiple Attribute Controlling}

\begin{table*}[t]
    \centering\footnotesize
    \tabcolsep=3pt
    \renewcommand\arraystretch{1.0}
    \begin{adjustbox}{max width=1\linewidth,width=0.95\linewidth,center=\linewidth}
    \begin{tabular}{r|ccccc|ccccc}
    \toprule
      \hspace{5.5mm}\multirow{4}{*}{\textbf{Model}} & \multicolumn{5}{c|} {\textbf{Double Controls}} & \multicolumn{5}{c}{\textbf{Triple Controls} } \\ \cmidrule{2-11}

    & Sent.($\uparrow$) & Top.($\uparrow$) & Ave.($\uparrow$) & PPL($\downarrow$) & Dist.($\uparrow$)& Sent.($\uparrow$) & Top.($\uparrow$) &Tense.($\uparrow$)  & PPL($\downarrow$) & Dist.($\uparrow$)\\
          \midrule
        
        \textsc{GeDi} & \textbf{99.47} & 51.36 &75.41 & 616.92 & \textbf{0.75}&
       -&-&-&-&-\\
       \textsc{Dist. Lens} &  77.47& 66.98 &72.22 & 52.59 & 0.26&
       65.31 &55.84 & 54.25 &63.13 & 0.40\\
        \textsc{Tailor} & 80.68 &68.72& 74.70 & 40.29 & 0.39&
        68.08 & 58.67&33.38 & 42.89 & 0.42\\
       \textsc{P-Gating} & 84.80 & \underline{75.02} & \underline{79.91} & \textbf{21.77} & 0.42&
        76.93 &62.73& 62.24 & 21.87 & 0.45\\
        % \textsc{PPO}  &  99.47 & 51.36 &75.41 & 616.92 & 0.75&
        % 76.10 & 73.80& 75.95 &116.6 & 0.75\\
        % \textsc{Quark}  &  99.47 & 51.36 &75.41 & 616.92 & 0.75&
        % 76.10 & 73.80& 75.95 &116.6 & 0.75\\
        \midrule
        \textsc{Tole} &  \underline{91.27} & \textbf{86.32} & \textbf{88.80} & \underline{38.62} & \underline{0.52} &
        \textbf{86.31} & \textbf{92.68}& \textbf{89.50} & \underline{40.75} & \underline{0.51}\\
        - weigher & 93.68 &78.72& 74.70 & 39.13 & 0.51&
        \underline{85.10} & \underline{84.72}& \underline{70.82} & 39.08 & 0.51\\
        
    \bottomrule
    \end{tabular}
    \end{adjustbox}
    \caption{Automatic evaluation results of the multi-attribute control task. Boldface and underline indicate the best two results.}
    \label{tab:multi-attribute}
\end{table*}

\textbf{Experimental Settings.} 
We conduct experiments on a double-attribute control task and a triple-attribute control task. We adopt the widely-used Yelp \cite{yelp} benchmark, containing restaurant reviews with the sentiment (positive and negative) and the subject (American, Mexican, and Asian) labels. To measure whether the sentence satisfies given attributes, we finetuned two RoBERTa-based \cite{roberta} classifiers for the evaluations of sentiment and subject with its original setting. Following \cite{prompt_gating}, we add another constraint, tense (past and present) \cite{tense} where their labels are automatically extracted from the reviews with an open-source toolkit\footnote{\url{https://github.com/ajitrajasekharan/simple_tense_detector}}.
%The cross-domain experiment uses the IMDb \cite{imdb} movie reviews for sentiment, and the AGNews dataset \cite{agnews} for topic. To evaluate the attribute accuracy, we use the classifiers trained by \cite{distributional} based on Deberta-v3 \cite{deberta}.
Perplexity (PPL) and averaged distinctness \cite{dist} are reported to demonstrate the fluency and diversity of the generated text. We also conduct human evaluations on generated results. Due to page limit, see Appendix \ref{apd:exp-multiple-attribute} for more details.

\textbf{Baselines.}
Research on multi-attribute CTG is not as abundant as single-attribute CTG. We extend
\textsc{GEDI} \cite{gedi}, which adopts a small-scale conditional generative discriminator to bias the token distribution, to multi-attribute controlling according to \citet{prompt_gating}. We also include \textsc{DIST. LENS} \cite{distributional}, which introduces an autoencoder to map constraints to latent subspaces, and explore the intersection of multiple constraints.
\textsc{Tailor} \cite{tailor} which proposes a connector to combine several prompts. Meanwhile, it modifies the attention mask and position indexes to narrow the gap between training and inference.
\textsc{Prompt-gating} \cite{prompt_gating}: it gates the prompts before appended into the LLMs to mitigate the mutual interference.
We also implement sentence-level RL methods,  PPO \cite{PPO} and Quark \cite{quark}, whose rewards are the sum of single-attribute rewards. We also conduct human evaluations. See Appendix \ref{apd:human} for more details.


\textbf{Results and Analysis.}
The results are shown in Table \ref{tab:multi-attribute}. The post-processing method, \textsc{GeDi}, though gets competitive results on attribute accuracy, the deterioration of text quality caused by direct decoding-time regulation is more severe than in single-attribute generation, indicated by the highest PPL score.
\textsc{Dist. Lens} though achieves considerable results, it requires over six times inference time to determine the intersection boundary of attribute subspaces.
Prompt-based methods \textsc{Tailor} and \textsc{Prompt-Gating} achieve suboptimal performance on both double- and triple-attribute scenarios. However, since they are easily overfitted to undesirable attributes in the training corpus which may contradict other target attributes, their performance is limited. With more fine-grained guidance on sampled sentences,
our method can achieve the best control accuracy in both settings without significant inference expenses.

\begin{figure}[tbp]
    \centering
    \includegraphics[width=\linewidth]{fig/noisechoice-acc.pdf}\\
    \includegraphics[width=\linewidth]{fig/noisechoice-dist.pdf}
    \caption{Performance of sentiment control with respect to training steps. "none" denotes the variance of no "quantize" nor "noise". "gauss." denotes the standard \textsc{Tole} with guassian noise. "sent." denotes the variance with sentence-level feedback.}
    \label{fig:withoutnoise}
\end{figure}


\subsection{Further Studies}
\label{sec:further_study}

\textbf{What effect do "Quantization" and "Noise" have respectively?} To visualize the difference made by "First quantize, then noise", we implement two variations of our algorithm, and conduct experiments on sentiment control tasks. 
First, we directly use the scores output by classifiers as rewards without any interference. We display the performance transition over the training steps of sentiment control tasks as in Figure \ref{fig:withoutnoise}. The figure demonstrates that the control accuracy and the text diversity both decrease. Our algorithm can achieve higher attribute accuracy since the noising procedure can promote the generalization of models, though initially converge slower. Moreover, the noising procedure can prevent models from flattering the scorers, thus achieving higher text diversity.
We also implement another variance that noise the reward without quantization boundaries.  
As shown in Figure \ref{fig:quantize-ablate}, we can see that quantization enhances the stability of algorithms. The model can learn from the relative order of datasets, even with a big standard deviation of Gaussian noise. If we ablate the quantization procedure, the algorithm will be sensitive to the amplitude of noise. 

\begin{figure}[tbp]
    \centering
    \includegraphics[width=0.49\linewidth]{fig/quantize-bar0.pdf}
    \includegraphics[width=0.49\linewidth]{fig/quantize-bar1.pdf}\\
    \includegraphics[width=0.49\linewidth]{fig/quantize-bar2.pdf}
    \includegraphics[width=0.49\linewidth]{fig/quantize-bar3.pdf}
    \caption{The performance comparison between model variances \textcolor{blue}{with} or \textcolor{red}{without} quantization procedure. The above two subgraphs are from neutral-to-positive experiments. The below are from detoxification.}
\label{fig:quantize-ablate}
\end{figure}

\textbf{What if we ablate the "weigher" from the multi-attribute combination, but adopt averages as overall rewards?} We implement a model variation that combines several scorers by averaging their output scores. Table \ref{tab:multi-attribute} shows that ablating "weigher" leads to a performance decrease. To further prove that "weigher" can provide more clear guidance with no contradiction between different scorers, we display the scores by averaging and aggregating by "weigher" respectively in Figure \ref{fig:ablateweigehr}. 
The left subgraph concentrate within small values due to the scorer contradiction without "weigher".
On the contrary, the right heatmap shows more distinct guidance for models.

\textbf{Convergence speed compared to sentence-level feedback.}
Token-level feedback can provide dense and precise signals for models, thus requiring fewer learning steps to achieve ideal performance. We implement a variance of \textsc{Tole} with sentence-level guidance with the same quantization \& noise process. We display the performance transition over training steps in Figure \ref{fig:withoutnoise}. The figure shows that the sentence-level feedback slows down the convergence significantly, compared to the token-level feedback.

\textbf{What effect does the number of quantiles have? }
$q$ of $q$-quantile does not have a significant effect on final performance. However, the convergence of the process is slightly slower if $q$ is relatively large or small. When $q$ is small, relative orders between quantiles are more ambiguous. A large $q$ confines noise within a small interval, diminishing noise impact, which results in a lower generalization. A moderate q-value allows the model to reach the desired result faster. See more details in Appendix \ref{apd:further-quantile-num}.


\textbf{What effect does the number of $\alpha,\beta$ have?}
$\alpha, \beta$ are two hyper-coefficients of KL-divergence and entropy term Eq.\ref{fml:loss_function} respectively. 
We conduct experiments with varying $\alpha,\beta$ of $0,0.05,0.1,0.15,0.2$. Experimental results indicate that higher $\alpha$ can increase text fluency, but sacrifice controllability slightly, since higher $\alpha$ more tightly constrain the model not to deviate too much.
Our experiments also demonstrate that the entropy term has a relatively slight effect on performance, not as much as KL-divergence. As $\beta$ increases, attribute accuracy and text diversity have a slight increase.
See more details in Appendix \ref{apd:coefficient}.

\textbf{Discussion about reward hacking.} Though our algorithm achieves great results in the above experiments, we are concerned that reward hacking occurs in some scenarios when scorers are too simple for LLMs to find unintended shortcuts. 
% To avoid reward hacking, our algorithm can complicate scoring patterns by integrating other controls of semantic or text degeneration.
One solution to reward hacking is to complicate reward design, which is easy to implement in our algorithms by adding new constraints with weighers. 

%We incrementally add a PPL constraint in sentiment control tasks, which makes this task contain two constraints as a multi-attribute control task. This variance can achieve on-par performance while achieving higher text fluency. See more details in Appendix \ref{apd:further-reward-hacking}.

\begin{figure}[t!]
    \centering
    \includegraphics[width=0.49\linewidth]{fig/scores-0.pdf}
    \includegraphics[width=0.49\linewidth]{fig/scores-1.pdf}
    \caption{Final scores of generated samples in explorations. The left is the average of two classifiers. The right is aggregated by "weigher".}
    \label{fig:ablateweigehr}
\end{figure}

==> latex/sections/introduction.tex <==
\section{introduction}
\label{sec:introduction}
Large autoregressive language models (LLMs) trained on extensive corpus can generate high-quality texts. However, to satisfy real-world applications, making the generation more controllable is urgent. It is desired to enhance specific attributes of generated texts for practical needs (e.g. positive sentiment for psychological escort, formality for academic writing) \citep{apply-1,apply-2,pretrain} and reduce intrinsic defects of pre-trained language models (e.g. toxicity, repetition) \citep{toxic-1,toxic-2}. 
%However, the deficient interpretability \citep{interpretability} of deep neural networks makes it challenging to guarantee the controllability of language models.

% It is natural to retrain neural language models on domain-specific data \citep{CTRL,cocon}. However, since the parameter scales of large language models keep increasing, retraining is subject to computational overheads.  
% %to significant computational overheads.
% Some researchers focus on post-processing methods \citep{fudge,dexpert,gedi}, which control the generation by manipulating possibility distributions generated with a fixed LLM. %, rather than training the language models themselves.
% They generally draw support from a small-scale attribute discriminator to regulate the possibility distribution for decoding. 
% %Since language models are not trained integrally, and thus can 
% Hence these methods can hardly capture higher-dimensional features, which results in their limited controllability. % (e.g. parsing structure, fine-grained semantics).
% % auxiliary discriminators can hardly adjust higher-order features such as syntax structure through the frozen language model,
% % However, due to the direct operations on generated probability distributions, post-processing methods cannot make language models understand high-order features within the text.
% %, which may also destroy the syntactic structure.
% %Some researches build small-scale attribute discriminators to adjust the next-token distribution based on the Bayesian rule. However, these methods convert the generation problem into a classification problem, which hinders language models from capturing high-order features in texts of certain attributes. However, the multiplications of two probability distributions make the language model lose insight into texts of certain attributes and destroy the syntactic structure. 
% Some researchers finetune the language models with partial parameters \citep{discup,tailor,contrast_prompt}, usually with continuous-prompt techniques \citep{continuous_prompt}.
% %to reduce computational expense while maintaining the potential of capturing high-dimensional features. 
% However, they generally require additional domain-specific corpus. Moreover, with a supervised training schema, models are easily overfitted to the unwanted aspects beyond the required attribute and suffer from the discrepancy between training and inferring known as exposure bias \citep{exposure_bias}.

Retraining models \cite{cocon,ctrl} are subject to computational overheads as the parameter scales become huge.
Post-processing methods \cite{gedi,fudge,dexpert} leverage small-scale discriminators to bias token distribution, which often leads to low text quality.
Some methods \cite{discup,tailor,prompt_gating} adopt parameter-efficient training strategy e.g. prefix-tuning, but they are susceptible to undesired attributes in the supervised corpus.
Recent research \cite{diffusionlm,distlens,normal_flow} introduces other algorithm backbones e.g. diffusion models, normalized flow, but they generally cost more computational expenses during trainig, and have a longer inference time, thus hard to deploy in real applications.


There is some research \cite{distributional,quark} introducing reinforcement learning (RL) into controllable text generation (CTG) tasks. 
RL paradigms can relieve the above problems, which alleviate the overfitting issue by training on self-generated sentences, and can integrate parameter-efficient strategies with canonical LLM backbones.
%Training language models on self-generated sentences can alleviate the above problems, which suits the reinforcement learning (RL) paradigm. 
%High-dimensional networks of RL models ensure the ability to capture high-level features, and the training corpus that comes from the RL models themselves alleviates the overfitting issue and exposure bias. 
%In natural language processing (NLP), Reinforced learning schemas \citep{PPO,REINFORCE} have been applied in many downstream tasks like relation extraction \citep{relation-extract1}, summarization \citep{summarization1,summarization2}, etc. and nowadays used at scale to tame the pre-trained language models with human feedback \citep{instructgpt}. 
However, RL-based methods generally update language models with sentence-level (or paragraph-level) rewards, leading to suboptimal performance and slow convergence. 
%However, RL feedback in NLP scenarios is generally sentence-level (or paragraph-level), since only after generating a complete sentence/paragraph can we score the text in previous settings. 
The coarse-grained rewards cannot provide clear guidance, since semantic in the sentence often transits with twists or progression. 
% Meanwhile, a sentence often contains irrelevant phrases and functional components for syntax.
Moreover, different parts of the sentence may contribute to different attributes.
Therefore, RL methods with coarse-grained feedback generally require considerable training steps to converge.

%It leads us to ponder whether we can propose finer-grained feedback to control the generation. %This is also consistent with intuitions since some parts of texts are only for the syntax completeness or semantic transition without any informativeness. 
%Existing RL-based methods generally train the networks with sentence-level labels as rewards. However, the various parts of the sentence contribute differently to a certain attribute. 
% It is also consistent with intuitions, for example, in the restaurant review "I'm overwhelmed by the delicious food lol!", the adjective "delicious" is the most critical in determining that the sentence is of positive sentiment, and the abbreviations "'m", "lol" indicate the informality the most. %换个例子？
%todo 这一段后续加上具体的指定节数。中间有的表述可能要替换。
%However, how to propose a reasonable mechanism to discriminate the importance of different textual tokens and suffice it to be extended to diverse control requirements is non-trivial. 
%Many prior works appoint sentence heuristics e.g. BLEU, Dist-n as rewards. Direct deconstructing this one-shot reward is impractical.
% Canonical decomposing methods such as Monte Carlo methods lead to a huge overhead of both time and storage in NLP scenarios since the action space of text generation is substantially large (\S\ref{sec:RL_formulation}), thus we cannot afford to enumerate enough cases to calculate the reward expectancy for each step. 
%Moreover, since the action space is substantially large (\S\ref{sec:RL_formulation}) in NLP scenarios, fine-grained control often requires value approximations to reduce computational overheads, which leads to a trade-off between value accuracy and training stability. This trade-off makes the RL training, which is known to be difficult to converge, even more unstable (\S\ref{sec:exp-further}). %which significantly encumbers the model performance. 

%This forces us to figure out how to get more accurate reward approximations while minimizing the computational overhead and how to maintain training stability while exploiting signals with noise. 

Our objective is to granularize the coarse-grained feedback to provide more precise guidance for LLMs. 
In this paper, we propose a novel reinforcement learning algorithm with \textbf{TO}ken-\textbf{LE}vel guidance named \textbf{TOLE}.
% We first transfer attribute scorers which provide coarse-grained rewards in prior methods to the token level with its sequential difference. 
We first provide an alternative perspective of Bayesian Factorization, which inspires us to formulate the token-level rewards as the probability shifts of attribute classifiers.
%The sequential difference indicates the contribution of the generated token, compared with the preceding subsentence. 
To enhance the robustness of TOLE, we propose an exploration framework with "First quantize, then noise" procedure. 
Moreover, TOLE can be extended to multi-attribute scenarios with few computational overheads. 
We conduct two experiments on single-attribute: sentiment control and detoxification. We also evaluate TOLE on multi-attribute scenarios with two settings. 
TOLE achieves superior performance compared with a wide range of baselines. 















==> latex/sections/methods.tex <==
\begin{figure*}
    \centering
    \includegraphics[width=\linewidth]{fig/colorful-framework1.pdf}
    \caption{Overall Framework of our algorithm.}
    \label{fig:enter-label}
\end{figure*}

\section{Approach}

We will first establish the notation, provide some background on existing RL methods in controllable text generation and model alignment, and offer an overview of our algorithm.

\subsection{Preliminaries}
\label{sec:RL_formulation}
\textbf{Notations.} A standard Markov Decision Process (MDP) can be denoted as $(\mathcal{S},\mathcal{A},\mathcal{T},r )$. At each step, an action $a \in \mathcal{A}$ is made based on the current state $s\in \mathcal{S}$. Then the state will be transited to $s'$ with the possibility $\mathcal{T}(s'|s,a)$. A function $r: \mathcal{S}\times\mathcal{A} \rightarrow \mathbb{R}$ defines the returned reward based on the states and actions. The strategy is decided by a policy model $\pi(\cdot|s)$, which is a predicted distribution over actions based on state $s$.
To transfer to text generation scenarios, the state can be defined as the partially generated sentence $y_{\leq i-1}=(y_1,y_2,\dots,y_{i-1})$, and the action is the next token $y_i \in \mathcal{V}$ where the vocabulary $\mathcal{V}$ is the action space. The transition dynamic $\mathcal{T}(\cdot|s,a)$ is deterministic since each state-action pair $(y_{\leq i-1},y_i)$ leads to a unique state $y_{\leq i}$. 
%The policy model is often a pre-trained LLM.

%\textbf{Feedback of RL in RLHF.} Distinct from CTG methods, RL methods of aligning LLMs often train a reward model to stimulate human feedback. This reward-learning procedure requires pairwise responses $y_h,y_l$ of the same instruction $x$, where $y_h,y_l$ are preferred and dispreferred responses respectively. Though there have been some concurrent efforts about token-level guidance in RLHF, they are still confined to the pairwise dataset settings. 

\textbf{Prior RL-based methods.} In previous RL-based methods of controllable text generation, rewards are derived from $\mathcal{P}(c|y)$, which denotes the possibility that the sentence $y$ satisfy the attribute $c$. $\mathcal{P}(c|y)$ can be obtained by corresponding attribute classifiers. 
%Scorers can be proxied diversely, e.g., retrained classifiers, off-shelf classifiers, and heuristic metrics. Though this setting has a great extensibility, prior research only concentrates on sentence-level feedback in single-aspect CTG. Directly transferring scorers into token-level guidance or combining several scorers for multi-aspect CTG will raise several problems.
Since prior research only concentrates on sentence-level feedback, which can be regarded as $r(y_1,y_{\leq 0})=r(y_2,y_{\leq 1})=\dots=r(y_{n+1},y_{\leq n})=f(\mathcal{P}(c|y))$. This equality means that sentence-level feedback treats each action $y_i$ in the MDP process of $y$ equally, which can only provide rough guidance for models.

\textbf{Bayesian Factorization in Prior research.} The objective of controllable text generation is to let LLMs approach $\mathcal{P}(y|c)$ where $c$ is a target attribute. Granularize to the token-level, prior post-processing methods generally factorize this term by the Bayesian formula as follows, 
\begin{equation}
    \mathcal{P}(y_{\leq i}|c) \propto \mathcal{P}(c|y_{\leq i})\mathcal{P}(y_i|y_{\leq i-1}).
\end{equation} 
With this formula, post-processing methods can achieve $\mathcal{P}(y|c)$ by regulating the token distribution $\mathcal{P}(y_i|y_{\leq i-1})$ with an attribute classifier which approximates $\mathcal{P}(c|y_{\leq i})$.

% In previous works \citep{quark,distributional}, rewards are generally returned after a whole sentence $y_{\leq L}$ is generated. They generally make the final feedback on behalf of the entire process and learn the entire trajectories of high-reward examples, which can be considered that action feedbacks from the same sentence are equal, formulated as $r(y_{\leq i-1},y_i)= f(y_{\leq L},c), i\in[1, L],$ where $f(y_{\leq L},c)$ is a scorer, rating how well the current sentences $y_{\leq L}$ match the requirement $c$. This estimation limits the model performance and slows down the convergence speed as shown in our experiments \S\ref{sec:exp-further}.


%\subsection{Novel RL Algorithm with Token-level Rewards}

\subsection{Token-level Rewards}

We first provide an alternative perspective of Bayesian factorization to show that the probability shift of attribute classifiers plays an important role in controlling the generations.
%If we transform the attribute condition $c$ to $c$ which means satisfying the given attribute $c$ when the current sentence is completed, 
The Bayesian factorization can be rewritten as:
\begin{equation}
    \mathcal{P}(y_i|y_{\leq i-1},c) 
    \propto \frac{\mathcal{P}(c|y_{\leq i})}{\mathcal{P}(c|y_{\leq i-1})}
    \mathcal{P}(y_i|y_{\leq i-1}).
\label{fml:newb}
\end{equation}
%, e.g., $\mathcal{P}(c_i|y_{\leq i-1})$ denotes the possibility of when the sentence $y_{\leq i-1}$ generates the next token, how likely the given attribute $c$ is satisfied. 是否需要这段例子解释?
%The detailed derivation, differences compared to the canonical form and the application of prior Bayesian factorization in previous works can be seen in Appendix \ref{apd:bayes}. 
See more details in Appendix \ref{apd:bayesian}. In Eq.\ref{fml:newb}, $\frac{\mathcal{P}(c|y_{\leq i})}{\mathcal{P}(c|y_{\leq i-1})}$ is crucial for the next-token probability distribution. Even if $y_{\leq i}$ tends to highly satisfy the condition $c$ when sentence is finished i.e. $\mathcal{P}(c|y_{\leq i})$ is large, action $y_i$ may not play an important role since previous $y_{\leq i-1}$ may already make future generations satisfy $c$ easily i.e. $\mathcal{P}(c|y_{\leq i-1})$ is large. It reveals that what matters is the probability shift between them, which enlightens our reward design. 

% To distinguish critical tokens from original sentences, previous sentence-level scorers should be converted into word level. 
The token-level reward function can be formulated as the probability shift before and after the word is generated.
\begin{equation}
    r(y_{i+1},y_{\leq i}) = f(\mathcal{P}(c|y_{\leq i+1}) - \mathcal{P}(c|y_{\leq i})),
\label{fml:token-level reward}
\end{equation}
% where $\mathcal{P}(c|y_{\leq i})$ is the probability that the sentence $y$ satisfy the attribute $c$ when the subsentence $y_{\leq i}$ completes.
where $f(\cdot)$ is an activation function for normalization, where we adopt the sigmoid function for implementations.
Theoretically, to approximate $\mathcal{P}(c|y_{\leq i})$, the format of training data should be transformed from the traditional $\{(y,c)\vert y\in \mathcal{Y}\}$ to $\{(y_{\leq i},c)\vert 0\leq i\leq |y|, y\in \mathcal{Y}\}$ as in \citet{fudge}. However, we find using traditional classifiers in our algorithms can achieve on-par performance in experiments compared to specially trained classifiers. We present this comparison in Appendix \ref{apd:further-fudge}.


\subsection{RL Algorithm: First quantize, then noise.} 
The training procedure of our RL algorithm can be separated into initialization, exploration, quantize \& noise, and learning. 
%Distinctively, the reward arrangement of our exploration procedure can be encapsulated as "First quantize, then noise". 
%The overall framework is shown in Figure \ref{fig:FIRE_framework} with an example from the sentiment control task. The formulaic algorithm is shown in Appendix \ref{apd:algorithm1}. 

\textbf{Initialization.} First, we initialize a policy LLM $\pi_\theta$, a copy of the policy model as the reference model $\pi_\textrm{ref}$, an attribute scorer $S$. The reference model is frozen during the whole process. We also initialize a data pool $\mathcal{D}=\varnothing$, and prepare a prefix corpus for exploration. 
%Since our fine-grained reward can guide the model more accurately, the exploration scale can be much smaller, thus less prepared corpus is required than previous RL methods for controllable generations.  

\textbf{Exploration.} Then, given the prefix $x$, the current policy model can generate subsequent text $y$. 
%The output logits are recorded for KL-divergence and entropy, and score intermediate state with nucleus sampling as in Eq.\ref{fml:final_state} to derive rewards as in Eq.\ref{fml:reward}. 
%When grading the sentences with an attribute discriminator $f(y,c)$ for state values, we adopt top-p sampling from the distribution of next-k tokens as in Eq.\ref{fml:final_state}.  
For each generated token, we calculate the score shift as its reward $r(y_{i+1},y_{\leq i})$, and add $(y_{i+1},y_{\leq i},r)$ to the data pool $\mathcal{D}$. 
To avoid over-training on data explored in earlier episodes, we set a lifetime for each data to indicate the episodes it can still undergo. Once the data is added to $\mathcal{D}$, the lifetime is initialized to $\mathcal{L}$ and subtracts 1 after each training episode. The data is removed from $\mathcal{D}$ when its lifetime drops to 0.

\textbf{Quantize \& Noise}
Learning primitive rewards $r$ can predispose the model to flatter the scoring pattern of attribute classifiers, which may cause diversity decrease. 
Therefore, we propose "First quantize, then noise" to avoid this problem.
First, we quantize the rewards within $\mathcal{D}$, and acquire $q$-quantiles, which divide the reward range into $q$ intervals. Then, we inject noise into each reward while ensuring each reward stays in the original interval. 
Specifically, for a reward $r \in (q_i,q_{i+1})$, we reassign it as 
\begin{equation}
    \hat{r}=q_i + (q_{i+1}-q_i)\epsilon(r-q_i) 
\label{fml:noise_reward}
\end{equation}
where $\epsilon(\cdot)$ is a noise processed with a clip function to satisfy $\epsilon(r) \in (r-1,r+1)$. $\epsilon(r)$ is substituted with Gaussian noise in our implementations.
Through this process, we disrupt the reward order to interfere the fixed scoring patterns of classifiers, while maintaining the relative order between intervals to steer LLMs toward the target attribute.

\textbf{Learning.} 
Through above procedures, we can obtain $\hat{r}$ to provide dense guidance on each token without granularity mismatch or feedback delay.
% In particular, a minimalist optimization problem can be formulated as follows:
% $$
% \max_\theta \mathbb{E}_{t\sim \textrm{Uniform}} \mathbb{E}_{y_{t+1}\sim \pi_\theta(\cdot|y_{\leq t})} \Big[ r(y_{t+1},y_{\leq t})\Big],
% $$
% where $\textrm{Uniform}$ is a uniform distribution among $\{0,\dots,|y|-1\}$.
The minimalist objective of our optimization problem is to maximize the total rewards, $
\max_\theta \mathbb{E}_{y_{t+1}\sim \pi_\theta(\cdot|y_{\leq t})} [ \hat{r}(y_{t+1},y_{\leq t}) ]
$.
We relax the convergence by adding a standard max-entropy gradient, which can help capture diverse behavior modes. We also insert a KL-divergence penalty to keep the model $\pi_\theta$ from deviating too far from the original $\pi_\textrm{ref}$. 
The gradient of each sentence $y$ can be formulated as follows,
\begin{equation}
\begin{aligned}
 &\mathbb{E}_{y_{t+1}\sim \pi_\theta(\cdot|y_{\leq t})} \Big[ \hat{r}(y_{t+1},y_{\leq t}) \nabla_\theta \log \pi_\theta(y_{t+1}|y_{\leq t}) \\
    &\qquad \qquad +\alpha\nabla_\theta  \mathcal{H}(\cdot|y_{\leq t}) + \beta\nabla_\theta  \textsc{KL}(y_{\leq t}) \Big]
\end{aligned}
\label{fml:loss_function}
\end{equation}
where $\alpha,\beta $ are two balancing coefficient, $\mathcal{H}$ is the Shannon entropy of $\pi_\theta(\cdot|y_{\leq t})$, $\textsc{KL}(y_{\leq t})$ is the KL divergence between $\pi_\theta(y_{t+1}|y_{\leq t})$ and $\pi_\textrm{ref}(y_{t+1}|y_{\leq t})$.


We then use the updated model for exploration and repeat the Exploration-Quantize \& Noise-Learning cycle until training achieves the maximum episode number.


% \textbf{Intuitive understanding of how FIRE works.}
% After parameters update in the previous episode, the current policy model becomes more likely to generate tokens whose rewards are higher than $r_h$, the $q$-quantile of rewards of examples within the data pool $\mathcal{D}$. Therefore, examples generated from the exploration of the current episode can be inferred to have a higher reward level compared to existing examples in $\mathcal{D}$. Inserting the upscale examples leads to a higher $q$-quantile $r_h^* > r_h$ of our training objective in the current episode. The policy model would learn from these more strictly screened samples, which leads to a higher $q$-quantile during the next exploration. Our model would gradually evolve by circulating this exploration-learning procedure.  

\subsection{Extension to Multiple Attributes.}
To consider multiple constraints simultaneously, we should combine multiple reward groups from different scorers. Simple aggregations or averages cannot provide appropriate token-level guidance, since scorers may contradict each other. Moreover, different parts of sentences may address different attributes, so we need to weigh the token's contribution to multiple attributes respectively.
To tackle this, we train a small-scale "weigher"  $W_\phi: \mathbb{R}^d \rightarrow \mathbb{R}^n$ to balance rewards from $n$ scorers, where $d$ is the hidden size of LLMs. 
Given the last-layer hidden states $\mathbf{H}_{t+1} \in \mathbb{R}^{1\times d}$ of $y_{t+1}$ output by LLMs $\pi(y_{\leq t+1})$, the weigher output $\mathbf{W} = W_\phi(\mathbf{H}_{t+1})$ as the weight for $n$ rewards of $y_t$, $\mathbf{R}_{t+1} \in \mathbb{R}^{1\times n}$. 
The weigher does not require a complex model structure. Simple structures can already assist our algorithm to achieve great performance. Hence it does not take significant computational overheads.
In our implementation, the weigher consists of two linear layers with the ReLU function and a output layer with a softmax function. 
The comprehensive reward of action $y_{t+1}$ can be obtained by $r = \mathbf{W}\times \mathbf{R}^T_{t+1}$.

To train the weigher, we formulate the optimization problem as maximizing the integrated reward of a training corpus $y\sim \mathcal{Y}$ that satisfies the multiple attributes,
\begin{equation}
    \max_\phi \mathbb{E}_{y \sim \mathcal{Y}}  \mathbb{E}_{t} W_\phi(\mathbf{H}_{t+1}) \times \mathbf{R}_{t+1}
\end{equation}
where $t\sim \textrm{Uniform}(0,|y|-1)$, a uniform distribution among $\{0,1,\dots,|y|-1\}$. By doing so, the weigher learns which scorer should be paid more attention when considering different tokens within sentences.

% \subsection{Theoretical Connection to Existing Policy-gradient RL}

% \textbf{Canonical policy-gradient RL.} 
% Review the training objective of the traditional policy-gradient RL methods \citep{REINFORCE} with baseline value,
% \begin{equation}
% \mathcal{r}_\theta \mathcal{J}(\theta) =  \mathbb{E} \Big[ \sum_{t=0}^{\infty} \big( G_t-b(s) \big)  \mathcal{r}_\theta \log {\pi(a_t|s_t,\theta)} \Big],
% \label{fml:origin_obj}
% \end{equation}
% where $G_t = \sum_{k=0}^\infty \gamma^k r_{t+k}$ is total amount of rewards obtained after step $t$ in the trajectory, and in our undiscounted RL setting $\gamma=1$. Prior research has shown that sole $G_t$ often leads to a high variance, hence they often substract a baseline value to stablize the training. This baseline is independent with action $a_t$, thus it would not disturb the overall expectile since $\mathbb{E}\big[b \mathcal{r}_\theta \log {\pi(a_t|s_t,\theta)} \big] = 0$. More details are shown in Appendix \ref{apd:theory1}. 

% \textbf{FIRE is a more conservative version of policy-gradient RL.}
% We derive the training objective of FIRE in Eq.\ref{fml:obj} to an analogous form of Eq.\ref{fml:origin_obj}. It indicates that FIRE is a more conservative version of canonical policy-gradient RL by clipping and reweighting. We present the derivation results as follows,
% \begin{equation}
% % \mathcal{r}_\theta \mathcal{J}(\theta) = \mathbb{E} \Big[ \sum_{n=0}^L \textsc{Clip}\Big( \lambda_n G_n - b(y_{\leq n})\Big) \mathcal{r}_\theta \log{\pi(y_{n+1}|y_{\leq n},\theta)} \Big],
% \mathcal{r}_\theta \mathcal{J}(\theta) = \mathbb{E} \Bigg[ \sum_{n=0}^L \Big[ \lambda_n
%     \textsc{Clip}^*\Big(  G_n - b(y_{\leq n})\Big) +1\Big] \mathcal{r}_\theta \log{\pi(y_{n+1}|y_{\leq n},\theta)} \Bigg]
% \label{fml:theory}
% \end{equation}
% where $b(y_{\leq n}) = \log (c_L|y_{\leq n})$ is the baseline value, $\lambda_n = \frac{1}{r_n}$ is a reweighting factor, $\textsc{Clip}(\cdot)$ is a clip function that masks values $a$ to 0 if $a<\textrm{threshold}$. The clipping function forces the gradient switches between the reweighted canonical gradient and 0 by a threshold corresponding to the highest $q$-quantile, which indicates that parameters only descend towards samples with high confidence. $\lambda_n$ is a reweighting factor to elude participation of precise reward value. Detailed derivations are shown in Appendix \ref{apd:theory2}.



==> latex/sections/related.tex <==
\section{Related Works}

\textbf{Controllable Text Generation.} Most previous works on controllable text generation (CTG) are based on the auto-regressive framework, which can be categorized into retraining \cite{ctrl,cocon}, finetuning \cite{prompt_gating,tailor,discup}, and post-processing \cite{gedi,dexpert,fudge}. Retraining and traditional finetuning methods are of low efficiency since the parameter scale of LMs is surging and the overfitting issue is severe. Post-processing methods regulate the next-token distribution with supplementary modules, mostly an attribute discriminator, but often cause syntax interruption and make language models lose insights. \citet{quark} integrate RL algorithms into CTG but use coarse-grained feedback to guide the LLMs.

\textbf{Multi-aspect controllable text generation.}
Along with single-aspect controlling, most research on multi-aspect controllable text generation can also categorized into finetuning and post-processing. Some post-processing research \cite{blend, mucoco} in MCTG combines multiple attribute discriminators to aggregate the controllability. However, they also inherit drawbacks of post-processing methods due to direct distribution regulations.
Finetuning-based research tries to connect several single controllers, e.g. connectors to combine multiple plugins \cite{tailor}, latent variables to represent the unsupervised aspects \cite{contrastive}, direct combination of prompts \cite{prompt_gating}, the boundary exploration of intersected subspaces \cite{distlens, normal_flow}. 
To the best of our knowledge, we are the first to explore how to extend single-attribute reinforcement learning algorithms to the MTCG scenario. 

\textbf{Token-level guidance for Reinforcement Learning.}
There is a series of research \citep{decision,rl_transformer1,rl_transformer2,rl_transformer3} incorporating RL techniques into the transformer structure, trying to deconstruct the coarse-grained reward into the token level for sequential modeling. However, they are hard to extend to practical applications since their specialized token settings are not in line with current LLMs.
Concurrent with our research, some research \cite{fine-grained-rlhf,token-level-rlhf} on LLM alignments tries to handle the problem of coarse-grained feedback. RLHF (reinforcement learning from human feedback) algorithms of the LLM alignment generally require a large-scale reward model, which should be trained on datasets formatted as pairwise sentences with the same prefix.
However, such data is unavailable when confronted with a wide variety of attribute requirements.
Therefore, exploring a novel reinforcement learning algorithm with token-level feedback is significant for controllable text generation.  

% Notably, concurrent to our research, the problem of coarse-grained feedback has also been identified in LLM alignment \cite{fine-grained-rlhf,token-level-rlhf}. 
% %However, alignment algorithms are not suitable for CTG tasks.
% However, alignment algorithms generally require a large-scale reward model trained on specialized datasets, formatted as pairwise sentences of the same prefix. 
% However, similar corpora are generally unavailable, let alone the extensibility for multi-attribute scenarios.
% %Moreover, in multi-aspect controllable text generation (MTCG), reward models should be retrained for every aspect combination on corpora with multi-aspect annotations. 
% Therefore, exploring a novel algorithm for token-level RL with high extensibility and non-restriction on data format is significant for controllable text generation.  
